Learning Audio-Visual embedding for Person Verification in the Wild

It has already been observed that audio-visual embedding is more robust than uni-modality embedding for person verification. Here, we proposed a novel audio-visual strategy that considers aggregators from a fusion perspective. First, we introduced weight-enhanced attentive statistics pooling for the first time in face verification. We find that a strong correlation exists between modalities during pooling, so joint attentive pooling is proposed which contains cycle consistency to learn the implicit inter-frame weight. Finally, each modality is fused with a gated attention mechanism to gain robust audio-visual embedding. All the proposed models are trained on the VoxCeleb2 dev dataset and the best system obtains 0.18%, 0.27%, and 0.49% EER on three official trial lists of VoxCeleb1 respectively, which is to our knowledge the best-published results for person verification.

==> tables/table_all.tex <==
\begin{table*}[htbp]
\vspace{-0.6cm}
\centering
\setlength{\tabcolsep}{1.5mm}
\caption{}
\label{tab:2}
%\resizebox{16cm}{45mm}
\scalebox{0.8}
{ 
\begin{threeparttable}
    \begin{tabular}{*{11}{c}}
      \toprule
      \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Type}}} &
      \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Architecture}}}\multirow{2}{*}
      & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{\#Modality}}} 
      & \multicolumn{2}{c}{\textbf{VoxCeleb1-O\tnote{$\dagger$}}} &
      \multicolumn{2}{c}{\textbf{VoxCeleb1-E\tnote{$\dagger$}}} &
      \multicolumn{2}{c}{\textbf{VoxCeleb1-H\tnote{$\dagger$}}} &\\ 
      \cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}
      & & & {\textbf{EER(\%)}} & {\textbf{MinDCF}} & {\textbf{EER(\%)}} & {\textbf{MinDCF}}& {\textbf{EER(\%)}} & {\textbf{MinDCF}}\\
      \midrule
       \multirow{3}*{None pretrain}&ECAPA-TDNN\cite{speaker_1} & A & 0.87 &  0.107 & 1.12 & 0.132 & 2.12  &0.210\\
        ~&SimAM-Resnet\cite{speaker_2} & A & 0.64 & 0.067  & 0.84 & 0.089 & 1.49  &0.146\\
        ~&MFA-Conformer\cite{speaker_3} & A & 0.64 & 0.081  & - & - & -  & -\\
      \midrule
      \multirow{4}*{\thead{Pretrain\\(only finetune classifier)}}&
        Hubert Base\cite{speaker_4,speaker_5} & A & 0.99 & - & 1.07 & - & 2.22 & -\\
        ~&Hubert Large\cite{speaker_4,speaker_5} & A & 0.81 & - & 0.82 & - & 1.68 & -\\
        ~&WavLM Base+\cite{speaker_4} & A & 0.84 & - & 0.93 & - & 1.76 & -\\
        ~&WavLM large\cite{speaker_4} & A & 0.62 & - & 0.67 & - & 1.32 & -\\
      \hline
      %\midrule
      \multirow{4}*{\thead{\makecell[c]{Pretrain\\(finetune pretrain modal\\and classifier)}}}
        &\multirow{2}*{\makecell[c]{Hubert Large\cite{speaker_4,speaker_5}}} & \multirow{2}*{A} & \multirow{2}*{0.59} & \multirow{2}*{-} & \multirow{2}*{0.65} & \multirow{2}*{-} & \multirow{2}*{1.34} & \multirow{2}*{-}\\
        ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~\\
        ~ &\multirow{2}*{\makecell[c]{WavLM large\cite{speaker_4}}} & \multirow{2}*{A} & \multirow{2}*{0.38} & \multirow{2}*{-} & \multirow{2}*{0.48}  & \multirow{2}*{-} & \multirow{2}*{0.99} & \multirow{2}*{-} \\
        ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~\\
      \midrule
       \multirow{12}*{Multimodal}&
          \multirow{4}*{Z. Chen\cite{Mult_ref_7}} 
           ~ & \ding{172}A & 2.308 & - & 2.234 & - & 3.782 & -\\
           ~& & \ding{173}V & 2.260 & - & 1.542 & - & 2.374 & -\\
            ~ & ~ & \ding{174}fusion & 0.585 & - & 0.427 & - & 0.735 & -\\
            ~ & ~ & ensemble(\ding{172},\ding{173}) & 0.505 & - & 0.432 & - & 0.782 & -\\
            ~ & ~ & ensemble(\ding{172},\ding{173},\ding{174}) & 0.499 & - & 0.379 & - & 0.683 & -\\
    \cmidrule(lr){2-9}
          &\multirow{3}*{Y. Qian\cite{Mult_ref_4}} 
           ~ & A & 1.62 & - & 1.75 & - & 3.16 & -\\
           ~& & V & 3.04 & - & 2.18 & - & 4.23 & -\\
            ~&~ & fusion & 0.71 & - & 0.48 & - & 0.85 & -\\
       %\multirow{4}*{Multimodal}&
        \cmidrule(lr){2-9}
     & \multirow{4}*{Ours} 
     ~ & \ding{175}A & 0.99 & 0.140 & 1.24 & 0.163 & 2.27 & 0.264\\
       ~& ~ & \ding{176}V & 1.44 & 0.147 & 1.28 & 0.157 & 2.14 & 0.230 \\
        ~&~ & fusion w/o cons\ddagger & 0.22 & 0.022 & 0.27 & 0.035 & 0.52 & 0.058\\
        ~&~ & \ding{177}fusion & 0.18 & 0.017 & 0.26 & 0.035 & 0.49 & 0.057\\
      \midrule
        Multimodal & Ours & ensemble(\ding{175},\ding{176},\ding{177}) & \textbf{0.14} & \textbf{0.012} & \textbf{0.21} & \textbf{0.028} & \textbf{0.37} & \textbf{0.046}\\
      \bottomrule
    \end{tabular}

    \begin{tablenotes}
    	\normalsize
    	\item[$\dagger$]Since 4 samples of the audio of voxceleb1 do not have corresponding images, the trials of these samples are eliminated in the visual and fusion task.
    	\item[$\ddagger$]"w/o cons" means "without cycle consistency learning".
    \end{tablenotes}

\end{threeparttable}
}
\vspace{-0.6cm}
\end{table*}


==> tables/table_all_small.tex <==
\begin{table*}[b]
\vspace{-0.6cm}
\centering
\setlength{\tabcolsep}{1.5mm}
\caption{\footnotesize
Performance of proposed network}
\label{tab:2}
%\resizebox{16cm}{45mm}
\scalebox{0.8}
{
\begin{threeparttable}
    \begin{tabular}{*{11}{c}}
      \toprule
      \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Type}}} &
      \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Architecture}}}\multirow{2}{*}
      & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{\#Modality}}} 
      & \multicolumn{2}{c}{\textbf{VoxCeleb1-O}} &
      \multicolumn{2}{c}{\textbf{VoxCeleb1-E}} &
      \multicolumn{2}{c}{\textbf{VoxCeleb1-H}} &\\ 
      \cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}
      & & & {\textbf{EER(\%)}} & {\textbf{MinDCF}} & {\textbf{EER(\%)}} & {\textbf{MinDCF}}& {\textbf{EER(\%)}} & {\textbf{MinDCF}}\\
      \midrule
       \multirow{2}*{Unimodal}&ECAPA-TDNN\cite{speaker_1} & A & 0.87 &  0.107 & 1.12 & 0.132 & 2.12  &0.210\\
        ~&SimAM-Resnet\cite{speaker_2} & A & 0.64 & 0.067  & 0.84 & 0.089 & 1.49  &0.146\\
        % ~&MFA-Conformer\cite{speaker_3} & A & 0.64 & 0.081  & - & - & -  & -\\
    %   \midrule
    %   \multirow{4}*{\thead{Pretrain\\(only finetune classifier)}}&
    %     Hubert Base\cite{speaker_4,speaker_5} & A & 0.99 & - & 1.07 & - & 2.22 & -\\
    %     ~&Hubert Large\cite{speaker_4,speaker_5} & A & 0.81 & - & 0.82 & - & 1.68 & -\\
    %     ~&WavLM Base+\cite{speaker_4} & A & 0.84 & - & 0.93 & - & 1.76 & -\\
    %     ~&WavLM large\cite{speaker_4} & A & 0.62 & - & 0.67 & - & 1.32 & -\\
    %   \hline
    %   %\midrule
    %   \multirow{4}*{\thead{\makecell[c]{Pretrain\\(finetune pretrain modal\\and classifier)}}}
    %     &\multirow{2}*{\makecell[c]{Hubert Large\cite{speaker_4,speaker_5}}} & \multirow{2}*{A} & \multirow{2}*{0.59} & \multirow{2}*{-} & \multirow{2}*{0.65} & \multirow{2}*{-} & \multirow{2}*{1.34} & \multirow{2}*{-}\\
    %     ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~\\
    %     ~ &\multirow{2}*{\makecell[c]{WavLM large\cite{speaker_4}}} & \multirow{2}*{A} & \multirow{2}*{0.38} & \multirow{2}*{-} & \multirow{2}*{0.48}  & \multirow{2}*{-} & \multirow{2}*{0.99} & \multirow{2}*{-} \\
    %     ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~\\
      \midrule
       \multirow{12}*{Audio-visual}&
          \multirow{4}*{Z. Chen\cite{Mult_ref_7}} 
           ~ & \ding{172}A & 2.308 & - & 2.234 & - & 3.782 & -\\
           ~& & \ding{173}V & 2.260 & - & 1.542 & - & 2.374 & -\\
            ~ & ~ & \ding{174}fusion & 0.585 & - & 0.427 & - & 0.735 & -\\
            ~ & ~ & ensemble(\ding{172},\ding{173}) & 0.505 & - & 0.432 & - & 0.782 & -\\
            ~ & ~ & ensemble(\ding{172},\ding{173},\ding{174}) & 0.499 & - & 0.379 & - & 0.683 & -\\
    \cmidrule(lr){2-9}
          &\multirow{3}*{Y. Qian\cite{Mult_ref_4}} 
           ~ & A & 1.62 & - & 1.75 & - & 3.16 & -\\
           ~& & V & 3.04 & - & 2.18 & - & 4.23 & -\\
            ~&~ & fusion & 0.71 & - & 0.48 & - & 0.85 & -\\
       %\multirow{4}*{Multimodal}&
        \cmidrule(lr){2-9}
     & \multirow{4}*{Ours} 
     ~ & \ding{175}A & 0.99 & 0.140 & 1.24 & 0.163 & 2.27 & 0.264\\
       ~& ~ & \ding{176}V & 1.44 & 0.147 & 1.28 & 0.157 & 2.14 & 0.230 \\
        ~&~ & fusion w/o cons$\dagger$ & 0.22 & 0.022 & 0.27 & 0.035 & 0.52 & 0.058\\
        ~&~ & \ding{177}fusion & 0.18 & 0.017 & 0.26 & 0.035 & 0.49 & 0.057\\
      \midrule
        Audio-visual & Ours & ensemble(\ding{175},\ding{176},\ding{177}) & \textbf{0.14} & \textbf{0.012} & \textbf{0.21} & \textbf{0.028} & \textbf{0.37} & \textbf{0.046}\\
      \bottomrule
    \end{tabular}

    \begin{tablenotes}
    	\normalsize
    % 	\item[$\dagger$]Since 4 samples of the audio of voxceleb1 do not have corresponding images, the trials of these samples are eliminated in the visual and fusion task.
    	\item[$\dagger$]"w/o cons" means "without cycle consistency learning".
    \end{tablenotes}

\end{threeparttable}
}
\vspace{0cm}
\end{table*}


==> tables/table_tanh_split.tex <==
% l 左 c 居中 r 对齐
% | 竖线 \hline横线 || 双竖线 \hline \hline 双横线
\vspace{-0.6cm}
\begin{table}[bhp]
\centering
%\small
\setlength{\tabcolsep}{0mm}
\caption{\footnotesize
Ablation study on activation}
\label{tab:1}
\resizebox{\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{*{10}{c}}
      \toprule
      \multicolumn{1}{c}{\multirow{2}{*}{\textbf{\#Modality}}}
      & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Architecture}}} 
      & \multicolumn{2}{c}{\textbf{Vox1-O\footnotemark[1]}} &
      \multicolumn{2}{c}{\textbf{Vox1-E\footnotemark[1]}} &
      \multicolumn{2}{c}{\textbf{Vox1-H\footnotemark[1]}} &\\
      \cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}
      & & {\textbf{\thead{EER(\%)}}} & {\textbf{\thead{MinDCF}}} & {\textbf{\thead{EER(\%)}}} & {\textbf{\thead{MinDCF}}}& {\textbf{\thead{EER(\%)}}} & {\textbf{\thead{MinDCF}}} & \\
      \midrule
      \multirow{4}*{V} 
      ~& Y. Qian\cite{Mult_ref_4} & 3.04 &  - & 2.18 & - & 4.23  & -\\
      ~&Z. Chen\cite{Mult_ref_7} & 2.26 & - & 1.54 & - & 2.37 & -\\
      ~&Ours(w/o)\dagger & 2.59 & 0.214 & 1.88 & 0.198 & 3.39 & 0.297\\
      ~&Ours & \textbf{1.44} & \textbf{0.147} & \textbf{1.28} & \textbf{0.157} & \textbf{2.14} & \textbf{0.230}\\
      \midrule
      \multirow{3}*{A} 
        ~&ECAPA-TDNN\cite{speaker_1} & 0.87 &  0.107 & 1.12 & 0.132 & 2.12  &0.210\\
        ~&Ours(w/o)\dagger$*$ & \textbf{0.98} & 0.140 & 1.24 & 0.163 & 2.30 & 0.264\\
        ~&Ours & 0.99 & 0.140 & \textbf{1.22} & \textbf{0.161} & \textbf{2.27} & 0.264\\
    \bottomrule
    \end{tabular}
    
    \begin{tablenotes}
    	\small
    	%\item[$\dagger$] Since 4 samples of the audio of voxceleb1 do not have corresponding images, the trials of these samples are eliminated in our own experiment.
    	\item[$\dagger$] "w/o" means "without tanh encoding"
    	\item[$*$] The gap between ours and ECAPA-TDNN in \cite{speaker_1} is mainly caused by the data augmentation method and dataset differences which will not affect the overall results in general.
    % 	\item[$*$]Upper part of the table is about single modality visual, lower part of the table is about single modality audio
    \end{tablenotes}
\end{threeparttable}
}
\vspace{-0.3cm}
\end{table}
\footnotetext[1]{Since 4 samples of the audio of VoxCeleb1 do not have corresponding images, the trials of these samples are eliminated in our own experiment.}
